HUGS: Human Gaussian Splats

Recent advances in neural rendering have improved both training and rendering times by orders of magnitude. While these methods demonstrate state-of-the-art quality and speed, they are designed for photogrammetry of static scenes and do not generalize well to freely moving humans in the environment. In this work, we introduce Human Gaussian Splats (HUGS) that represents an animatable human together with the scene using 3D Gaussian Splatting (3DGS). Our method takes only a monocular video with a small number of (50-100) frames, and it automatically learns to disentangle the static scene and a fully animatable human avatar within 30 minutes. We utilize the SMPL body model to initialize the human Gaussians. To capture details that are not modeled by SMPL (e.g. cloth, hairs), we allow the 3D Gaussians to deviate from the human body model. Utilizing 3D Gaussians for animated humans brings new challenges, including the artifacts created when articulating the Gaussians. We propose to jointly optimize the linear blend skinning weights to coordinate the movements of individual Gaussians during animation. Our approach enables novel-pose synthesis of human and novel view synthesis of both the human and the scene. We achieve state-of-the-art rendering quality with a rendering speed of 60 FPS while being ~100x faster to train over previous work. Our code will be announced here: https://github.com/apple/ml-hugs

==> figures/qual_demo.tex <==
% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/pdf_files/qual_demo.pdf}
%     \caption{Canonical pose left, novel view animation right} 
%     \label{fig:qual_demo}
%     \vspace{-2ex}
% \end{figure*}{}

==> figures/supmat_teaser.tex <==
\twocolumn[{%
	\renewcommand\twocolumn[1][]{#1}%
	\maketitle
	\begin{center}
		\newcommand{\teaserwidth}{\textwidth}
		% \vspace{-0.15in}
		\centerline{
			\includegraphics[width=\teaserwidth,clip]{figures/pdf_files/teaser_v2.pdf}
		}
		\vspace{-1ex}
		\captionof{figure}{\textbf{Human Gaussian Splats (\acronym)} is a neural rendering framework that trains on 50-100 frames of a monocular video containing a human in a scene. HUGS enables novel view rendering with novel human poses at \textbf{60 FPS} by learning a disentangled representation that can also render the human in other scenes.  \textcolor{magenta}{\textbf{*}Main submission indicates runtime speed as 32 FPS. During SupMat submission we have found out a bug causing slow performance. After resolving the issue, actual speed becomes 60 FPS.} }
		% \vspace{-0.08in}
		\label{fig:teaser}
	\end{center}%
}]

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\newcommand{\bm}{}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/07_macros.tex <==
\newcommand{\acronym}{HUGS\xspace}
\newcommand{\rgb}{RGB\xspace}
\newcommand{\smpl}{\mbox{SMPL}\xspace}
\newcommand{\smplx}{\mbox{SMPL-X}\xspace}
\newcommand{\gauss}{3D Gaussians\xspace}
\newcommand{\gausssplat}{3D Gaussian splatting\xspace}
\newcommand{\nerf}{NeRF\xspace}
\newcommand{\gstd}{3D Gaussian Splatting\xspace}

\newcommand{\vect}[1]{\mathbf{#1}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}

\newcommand{\shapecoeff}{\bm{\beta}}
\newcommand{\shapedim}{{\left| \shapecoeff \right|}}
\newcommand{\shapespace}{\mathcal{S}}
\newcommand{\shapespaceexpl}{\mathbb{R}^{\shapedim}}

\newcommand{\numjoints}{n_k}
\newcommand{\joints}{{J}}
\newcommand{\jointregressor}{\mathcal{J}}

\newcommand{\posecoeff}{\bm{\theta}}
\newcommand{\posedim}{{3\numjoints+3}}
\newcommand{\posespace}{\mathcal{P}}
\newcommand{\posespaceexpl}{\mathbb{R}^{\posedim}}

\newcommand{\expcoeff}{\bm{\psi}}
\newcommand{\expdim}{{\left| \expcoeff \right|}}
\newcommand{\expspace}{\mathcal{E}}
\newcommand{\expspaceexpl}{\mathbb{R}^{\expdim}}

\newcommand{\numverts}{n_v}
\newcommand{\numfaces}{n_t}
\newcommand{\template}{\bar{\bm{T}}}

\newcommand{\blendweight}{w}
\newcommand{\blendweights}{\mathcal{W}}
\newcommand{\blendweightsdim}{\left| \numjoints \times \numverts \right|}
\newcommand{\lbs}{\text{LBS}}

\newcommand{\verts}{\mathbf{V}}
\newcommand{\faces}{\mathbf{F}}
\newcommand{\vsmplx}{M}
\newcommand{\matsmplx}{\mathbf{M}}
\newcommand{\offsets}{{O}}
\newcommand{\offset}{\bm{o}}

\newcommand{\offsetmodel}{{F_{d}}}
\newcommand{\texmodel}{{F_{t}}}
\newcommand{\clothmodel}{{F_{c}}}
\newcommand{\defmodel}{{F_{e}}}

\newcommand{\image}{I}
\newcommand{\imagemask}{S} %
\newcommand{\numframes}{n_f}

\newcommand{\numsamples}{n_s}




\newcommand{\openpose}{\mbox{OpenPose}\xspace}
\newcommand{\cuda}{\mbox{CUDA}\xspace}
\newcommand{\pytorch}{\mbox{PyTorch}\xspace}
\newcommand{\mocap}{\mbox{MoCap}\xspace}
\newcommand{\inthewild}{\mbox{in-the-wild}\xspace}
\newcommand{\twoD}{2D\xspace}
\newcommand{\threeD}{3D\xspace}
\newcommand{\sixD}{6D\xspace}

\newcommand{\supmat}{Sup.~Mat.\xspace}

%\crefname{section}{Sec.}{Secs.}
\Crefname{section}{Section}{Sections}
\Crefname{table}{Table}{Tables}
%\crefname{table}{Tab.}{Tabs.}

==> sections/08_smpl.tex <==
\subsubsection{SMPL parametric body model}

\smpl is a parametric body model which allows pose and shape control. A subject's body mesh in the rest pose is defined as
\begin{equation}
    T_P(\shapecoeff,\posecoeff, \expcoeff) = \template + B_{S}(\shapecoeff;\shapespace) +  B_{P}(\posecoeff;\posespace)
\end{equation}
where $\template \in \mathbb{R}^{\numverts \times 3}$ is a template of body shape in the rest pose, $\shapecoeff \in \shapespaceexpl$ is the body identity parameters, and $B_{S}(\shapecoeff;\shapespace): \shapespaceexpl \rightarrow \mathbb{R}^{\numverts \times 3}$ are the identity blend shapes. More specifically, $B_S(\shapecoeff;\shapespace)=\sum_{i=1}^{|\shapecoeff|}\shapecoeff_i\shapespace_i$ where $\shapecoeff_i$ is the $i$-th linear coefficient and $\shapespace_i$ is the $i$-th orthonormal principle component. $\posecoeff\in\posespaceexpl$ denotes the pose parameters. Similar to the shape space $\shapespace$, $B_{P}(\posecoeff;\posespace): \mathbb{R}^{|\posecoeff|} \rightarrow \mathbb{R}^{\numverts \times 3}$ denotes the pose blend shapes ($\posespace$ is the pose space) from the \smpl model.
To capture more geometric details, we use an upsampled version of \smpl with $\numverts=110,210$ vertices and $\numfaces=220,416$ faces.


\subsubsection{Pose-dependent Deformation} 
Given the monocular video, we need to model the movement of this subject. 
Since our initialized avatar is based on \smpl, it provides a good way to capture the pose deformation.
For each frame of given video, we estimate the \smpl parameters  $\posecoeff \in \mathbb{R}^{|\posecoeff|}$. 
Then we can deform the head/body to the observation pose using the linear blend skinning function (\ie, $\lbs$).  
The deformation for the explicit \smpl mesh model is modeled by a differential function $\vsmplx(\shapecoeff, \posecoeff, \expcoeff, \bm{O})$ that outputs a 3D human body mesh $(\bm{V},\bm{F})$ where $\bm{V}\in\mathbb{R}^{\numverts\times 3}$ is a set of $\numverts$ vertices and $\bm{F}\in\mathbb{R}^{\numfaces\times 3}$ is a set of $\numfaces$ faces with a fixed topology:
\begin{equation}
        \vsmplx(\shapecoeff, \posecoeff, \expcoeff, \bm{O}) =  \lbs(\tilde{T}_P(\shapecoeff, \posecoeff, \expcoeff, \bm{O}), \joints(\shapecoeff), \posecoeff, \bm{W}),
\end{equation}
in which $\thickmuskip=2mu \medmuskip=2mu \bm{W} \in \mathbb{R}^{\numjoints \times \numverts}$ is the blend skinning weights used in the $\lbs$ function. $\thickmuskip=2mu \medmuskip=2mu\joints(\shapecoeff)\in\mathbb{R}^{n_k\times 3}$ is a function of body shape~\cite{SMPL:2015}, representing the shape-dependent joints. Given a template vertex $\bm{t}_i$, the vertex $\bm{v}_i$ can be computed with simple linear transformation. Specifically, the forward vertex-wise deformation can be written as the following equation in the homogeneous coordinates:
\begin{equation}
\begin{aligned}
    \underbrace{\bm{v}_i}_{\textnormal{Posed vertex}} = \underbrace{\sum_{k=1}^{n_k}\bm{W}_{k,i}G_k(\bm{\theta},J(\bm{\beta}))\cdot
        \begin{bmatrix}
     \bm{I} &  \bm{o}_i+ \bm{b}_i \\
      \bm{0} &  1 
  \end{bmatrix}}_{\vsmplx_i(\bm{\beta},\bm{\theta},\bm{\psi},\bm{O})\textnormal{:~Deformation to the posed space}}\cdot\underbrace{\bm{t}_i}_{\textnormal{Template vertex}}\nonumber,
\end{aligned}
\end{equation}
% \begin{equation}
% \begin{aligned}
%     \underbrace{\bm{v}_i^h}_{\textnormal{Posed vertex}} = \underbrace{\sum_{k=1}^{n_k}\bm{W}_{k,i}G_k(\bm{\theta},J(\bm{\beta}))\cdot
%         \begin{bmatrix}
%      \bm{I} &  \bm{o}_i+ \bm{b}_i \\
%       \bm{0} &  1 
%   \end{bmatrix}}_{\vsmplx_i(\bm{\beta},\bm{\theta},\bm{\psi},\bm{O})\textnormal{:~Deformation to the posed space}}\cdot\underbrace{\bm{t}_i^h}_{\textnormal{Template vertex}}\nonumber,
% \end{aligned}
% \end{equation}
where $\vsmplx_i(\bm{\beta},\bm{\theta},\bm{\psi},\bm{O}) \in \mathbb{R}^{4\times 4}$ is the deformation function of template vertex $\bm{t}_i$.   
$\bm{W}_{k,i}$ is the $(k,i)$-th element of the blend weight matrix $\bm{W}$, $G_k(\bm{\theta},J(\bm{\beta}))\in\mathbb{R}^{4\times 4}$ is the world transformation of the $k$-th joint and $\bm{b}_i$ is the $i$-th vertex of the sum of all blend shapes $\bm{B} := B_S(\bm{\beta})+B_P(\bm{\theta})+B_E(\bm{\psi})$. We denote $\bm{V}$ as the vertex set of the posed avatar ($\bm{v}_i\in\bm{V}$). Both $\bm{v}_i$ and $\bm{t}_i$ are the homogeneous coordinates when applying this deformation function. 
% of the posed vertex $\bm{v}_i$ and the rest template vertex $\bm{t}_i$, respectively.









% from method (move to supplementary)

\paragraph{SMPL~\cite{SMPL:2015}} is a parametric body model which allows pose and shape control. 
%
A body mesh in the rest pose (\ie, T-pose) is defined as
%
\begin{equation}
    T_P(\shapecoeff,\posecoeff, \expcoeff) = \template + B_{S}(\shapecoeff;\shapespace) +  B_{P}(\posecoeff;\posespace),
\end{equation}
%
where $\template \, {\in} \, \mathbb{R}^{\numverts \times 3}$ is a template of body shape in the rest pose, 
%
$\shapecoeff \, {\in} \, \shapespaceexpl$ are the body identity parameters, 
%
and $B_{S}(\shapecoeff;\shapespace){:} \, \shapespaceexpl \, {\rightarrow} \, \mathbb{R}^{\numverts {\times} 3}$ is the identity blend shape.
%
% and $B_{P}(\posecoeff;\posespace){:} \, \mathbb{R}^{|\posecoeff|} \, {\rightarrow} \, \mathbb{R}^{\numverts {\times} 3}$ are the identity and pose blend shapes, respectively. 
%
Specifically, $B_S(\shapecoeff;\shapespace)=\sum_{i=1}^{|\shapecoeff|}\shapecoeff_i\shapespace_i$, where $\shapecoeff_i$ is the $i$-th element in $\shapecoeff$ and $\shapespace_i$ is the $i$-th orthonormal principle component of the shape space $\shapespace$. 
%
Similarly, $B_{P}(\posecoeff;\posespace){:} \, \mathbb{R}^{|\posecoeff|} \, {\rightarrow} \, \mathbb{R}^{\numverts {\times} 3}$ is the pose blend shape that is calculated by linearly combining the principle components of the pose space $\posespace$ with the pose parameters $\posecoeff \, {\in} \, \posespaceexpl$.
%
% To capture more geometric details, we use an upsampled version of \smpl with $\numverts \, {=} \, 110,210$ vertices and $\numfaces \, {=} \, 220,416$ faces.


%\paragraph{Pose-dependent Deformation.} 
%Given the monocular video, we need to model the movement of this subject. 
%Since our initialized avatar is based on \smpl, it provides a good way to capture the pose deformation.
%For each frame of given video, we estimate the \smpl parameters  $\posecoeff \in \mathbb{R}^{|\posecoeff|}$. 
%Then we can deform the head/body to the observation pose using the linear blend skinning function (\ie, $\lbs$).  
%
The deformation of the \smpl mesh model is modeled by a differentiable function $\vsmplx(\shapecoeff, \posecoeff)$ that takes the shape and pose parameters as input and outputs a 3D human body mesh $(\bm{V},\bm{F})$ with $\numverts$ vertices $\bm{V}\in\mathbb{R}^{\numverts\times 3}$  and  $\numfaces$ faces $\bm{F}\in\mathbb{R}^{\numfaces\times 3}$ with a fixed topology. 
%
It is given by
\begin{equation}
\vsmplx(\shapecoeff, \posecoeff) =  \lbs(\tilde{T}_P(\shapecoeff, \posecoeff), \joints(\shapecoeff), \posecoeff, \bm{W}),
\end{equation}
where $\bm{W} \, {\in} \, \mathbb{R}^{\numjoints {\times} \numverts}$ is the linear blend skinning weights, $\numjoints$ is the number of joints, the linear blend skinning ($\lbs$) function will be introduced below,  
$\joints(\shapecoeff)\, {\in} \, \mathbb{R}^{n_k {\times} 3}$ is a function of body shape~\cite{SMPL:2015}, representing the shape-dependent joints. Given a template vertex $\bm{t}_i$, the vertex $\bm{v}_i$ can be computed with simple linear transformation. Specifically, the forward vertex-wise deformation can be written as the following equation in the homogeneous coordinates:


\begin{equation}
\small
\begin{aligned}
    \underbrace{\bm{v}_i}_{\textnormal{Posed vertex}} = \underbrace{\sum_{k=1}^{n_k}\bm{W}_{k,i} \, G_k(\bm{\theta},J(\bm{\beta}))\cdot
        \begin{bmatrix}
     \bm{I} &  \bm{b}_i \\
      \bm{0} &  1 
  \end{bmatrix}}_{\vsmplx_i(\bm{\beta},\bm{\theta})\textnormal{:~Deformation to the posed space}}\cdot\underbrace{\bm{t}_i}_{\textnormal{Template vertex}},
\end{aligned}
\end{equation}
%
where $\vsmplx_i(\bm{\beta},\bm{\theta}) \, {\in} \, \mathbb{R}^{4 {\times} 4}$ is the deformation function of template vertex $\bm{t}_i$.   
$\bm{W}_{k,i}$ is the $(k,i)$-th element of the blend weight matrix $\bm{W}$, $G_k(\bm{\theta},J(\bm{\beta}))\in\mathbb{R}^{4\times 4}$ is the world transformation of the $k$-th joint and $\bm{b}_i$ is the $i$-th vertex of the sum of all blend shapes $\bm{B} := B_S(\bm{\beta})+B_P(\bm{\theta})+B_E(\bm{\psi})$. We denote $\bm{V}$ as the vertex set of the posed avatar ($\bm{v}_i\in\bm{V}$). Both $\bm{v}_i$ and $\bm{t}_i$ are the homogeneous coordinates when applying this deformation function. 
% of the posed vertex $\bm{v}_i$ and the rest template vertex $\bm{t}_i$, respectively.

==> sections/scratch.tex <==
Photorealistic rendering and animation of human bodies is an important area of research with many applications in AR/VR, visual effects, visual try-on, movie production, etc. Successful tools for creating human avatars should enable easy data capture, efficient computation, and create a photo-realistic and animatable representation of the subject human. Unfortunately, existing approaches fall short of meeting these requirements. Previous work~\cite{alexander2010emily, alexander2013digitalira} for creating human avatars relied on capturing high quality data in a multi-camera capture setup, extensive compute, and a lot manual effort.

Therefore, our goal is to enable photorealistic animatable avatar with minimal capture.. compute .. To this end, we formulate our problem as a neural rendering of ....
scenario where only one single video is provided, and our goal is to reconstruct the human model and the static scene model, and enable novel pose rendering of the human, without any expensive multi-cameras setups or manual annotations. 

What is the problem with the existing work?
Recent work on Neural Fields include NeRFs~\cite{mildenhall2020nerf}, MPI~\cite{}, Image-based rendering~\cite{IBR_stuff}, point-based rendering ~\cite{adop, pointersect, pulsar}. However, their ability to capture deformable entities such as humans, bodies etc is either too slow or too bad. 

%
Recent approaches for generating 3D avatars from videos can be categorized into two main approaches. The first approach~\cite{} builds upon 3D parametric body models like SMPL(-X)~\cite{}, which offers advantages such as efficient rasterization and the ability to adapt to unseen deformations. However, it has limitations when it comes to modeling individuals with clothing or intricate hairstyles due to the inherent constraints of template meshes, such as fixed topologies and surface-like geometries.

Alternatively, recent advancements have explored the use of neural field representations for modeling 3D human avatars~\cite{jiang2022neuman}. These neural implicit representations excel in capturing details like clothing, accessories, and hair, surpassing the capabilities of parametric body model-based techniques. However, they come with trade-offs, notably being less efficient to train and render. 
This inefficiency arises from the need to query numerous points along the camera ray to render a single pixel. 
Furthermore, deformation of neural fields in a versatile manner presents challenges, often requiring recourse to an inefficient root-finding loop, which adversely affects both training and rendering durations~\cite{}.

To address these challenges, we introduce a novel avatar representation \emph{\acronym\;-- Human Gaussian Splats}. \acronym employs a set of \gauss to represent the canonical geometry and learns how to deform \gauss for animation. Specifically, we optimize a set of 3D Gaussians to represent the human geometry in a canonical space. For animation, a forward deformation module transforms these canonical points into a deformed space, \st{utilizing learned pose blendshapes and skinning weights, guided by pose parameters from a pre-trained parametric body model like \smpl.}\ar{No need for details here, pose blendshapes/parameters have still not been introduced.}



In contrast to implicit representations, our approach based on \gauss allows for efficient rendering through a differentiable rasterizer~\cite{kerbl3Dgaussians}. Additionally, they can be deformed effectively using established techniques \eg linear blend skinning. Compared to meshes, 3D Gaussians exhibit greater flexibility and versatility. Furthermore, in contrast to point clouds, they do not result in holes in the final rendered images.  
\rick{isn't it inaccurate? maybe say it is a continuous representation so easier to optimize.}
%
Beyond their capacity to accommodate changes in topology to model accessories and clothing, they are also well-suited for representing intricate volumetric structures, including hair. Additionally, existing joint human and scene~\cite{jiang2022neuman, guo2023vid2avatar} novel view synthesis approaches use \nerf as their representation. They need to deal with ray warping and ray classification to correctly disentangle scene and human points. Our use of \gauss prevents this issue by rasterizing the scene and human \gauss jointly when obeying their respective depth. This results in much more accurate scene and human separation compared to existing works~\cite{jiang2022neuman,guo2023vid2avatar}.

% How do we solve it
We demonstrate that ... 
As demonstrated using various videos captured in the wild, the proposed representation combines the advantages of popular mesh, point-based and implicit representations, and surpasses both in many challenging scenarios. In summary, our contributions are:


   1. We propose a forward deformation module with 3D gaussians to learn a canonical human gaussian model.
   2. We perform joint optimization of scene and human gaussians to showcase the mutual benefit of joint optimization.
   3. We obtain state-of-the-art performance on NeuMan and ZJU-Mocap datasets while achieving realtime rendering speeds.


To address these issues, we propose HUGS, a novel animatable avatar representation that uses 3D Gaussians to represent the canonical geometry and learns how to deform 3D gaussians for animation. Specifically, we optimize a set of 3D gaussians to represent the geometry of a subject in a canonical space. For animation, a forward deformation module maps the canonical points to the deformed space with learned pose blendshapes and skinning weights, given pose parameters of a pretrained parametric body model \ie \smpl. Compared to implicit representations, our 3D Gaussians-based representation can be rendered efficiently with a standard differentiable rasterizer. Moreover, they can be deformed effectively using established techniques, \eg, skinning. Compared to meshes, 3D gaussians are considerably more flexible and versatile. And compared to point clouds, they do not suffer from holes in the final rendered images. Besides the ability to conform the topology to model accessories and clothing, they can also represent complex volume-like structures such as hair.

==> tables/neuman_ablation.tex <==
\begin{table*}[]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|ccc|ccc|ccc|ccc|ccc|ccc}
    \toprule
        & \multicolumn{3}{c|}{\textbf{Seattle}} & \multicolumn{3}{c|}{\textbf{Citron}} & \multicolumn{3}{c|}{\textbf{Parking}} & \multicolumn{3}{c|}{\textbf{Bike}} & \multicolumn{3}{c|}{\textbf{Jogging}} & \multicolumn{3}{c}{\textbf{Lab}}   \\
    \midrule
        & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$  \\
    \midrule
    w/o LBS             &                      25.80 &  \cellcolor{tabfirst}0.85 & \cellcolor{tabsecond}0.14 & \cellcolor{tabsecond}25.36 &  \cellcolor{tabfirst}0.86 &  \cellcolor{tabfirst}0.15 & \cellcolor{tabsecond}26.68 &  \cellcolor{tabfirst}0.85 & \cellcolor{tabsecond}0.23 &  \cellcolor{tabfirst}25.62 & \cellcolor{tabsecond}0.84 &  \cellcolor{tabfirst}0.13 &  \cellcolor{tabthird}23.70 &  \cellcolor{tabfirst}0.78 & \cellcolor{tabsecond}0.22 & \cellcolor{tabsecond}25.96 & \cellcolor{tabsecond}0.91 &  \cellcolor{tabfirst}0.09 \\
    \midrule
    w/o Densify         &                      25.52 &  \cellcolor{tabthird}0.83 &                      0.17 &                      21.65 & \cellcolor{tabsecond}0.83 & \cellcolor{tabsecond}0.19 &                      24.32 &  \cellcolor{tabthird}0.80 &                      0.31 & \cellcolor{tabsecond}25.61 &  \cellcolor{tabthird}0.83 &  \cellcolor{tabthird}0.16 &                      21.37 &  \cellcolor{tabthird}0.73 &                      0.26 &                      23.95 &  \cellcolor{tabthird}0.90 &  \cellcolor{tabthird}0.11 \\
    \midrule
    w/o $\mathcal{L}^h$ &  \cellcolor{tabfirst}26.34 &  \cellcolor{tabfirst}0.85 &  \cellcolor{tabfirst}0.13 &  \cellcolor{tabthird}24.60 &  \cellcolor{tabfirst}0.86 &  \cellcolor{tabfirst}0.15 &  \cellcolor{tabthird}25.48 &  \cellcolor{tabfirst}0.85 &  \cellcolor{tabthird}0.25 &  \cellcolor{tabfirst}25.62 &  \cellcolor{tabfirst}0.85 &  \cellcolor{tabfirst}0.13 &  \cellcolor{tabfirst}24.10 &  \cellcolor{tabfirst}0.78 &  \cellcolor{tabfirst}0.21 &  \cellcolor{tabthird}25.94 & \cellcolor{tabsecond}0.91 & \cellcolor{tabsecond}0.10 \\
    \midrule
    w/o Triplane        & \cellcolor{tabsecond}25.96 & \cellcolor{tabsecond}0.84 &  \cellcolor{tabthird}0.15 &                      21.93 & \cellcolor{tabsecond}0.83 & \cellcolor{tabsecond}0.19 &                      23.90 & \cellcolor{tabsecond}0.81 &                      0.30 &  \cellcolor{tabthird}25.49 & \cellcolor{tabsecond}0.84 & \cellcolor{tabsecond}0.15 &                      22.02 & \cellcolor{tabsecond}0.74 &  \cellcolor{tabthird}0.25 &                      22.65 &                      0.89 &                      0.12 \\
    \midrule
    HUGS                &  \cellcolor{tabthird}25.94 &  \cellcolor{tabfirst}0.85 &  \cellcolor{tabfirst}0.13 &  \cellcolor{tabfirst}25.54 &  \cellcolor{tabfirst}0.86 &  \cellcolor{tabfirst}0.15 &  \cellcolor{tabfirst}26.86 &  \cellcolor{tabfirst}0.85 &  \cellcolor{tabfirst}0.22 &                      25.46 & \cellcolor{tabsecond}0.84 &  \cellcolor{tabfirst}0.13 & \cellcolor{tabsecond}23.75 &  \cellcolor{tabfirst}0.78 & \cellcolor{tabsecond}0.22 &  \cellcolor{tabfirst}26.00 &  \cellcolor{tabfirst}0.92 &  \cellcolor{tabfirst}0.09
    \\ 
    \bottomrule
    \end{tabular}  
    }
    \caption{NeuMan Ablation experiments}
    \label{tab:neuman_ablation}
\end{table*}

==> tables/neuman_novel_view_table.tex <==

\begin{table}[t]
\begin{center}
\begin{tabular}{lccccccccc}
\toprule
          & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Seattle\end{tabular}}  & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Citron\end{tabular}}   & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Parking\end{tabular}} \\
          & \multicolumn{1}{c}{PSNR$\uparrow$} & \multicolumn{1}{c}{SSIM$\uparrow$} & \multicolumn{1}{c}{LPIPS$\downarrow$} & \multicolumn{1}{c}{PSNR$\uparrow$} & \multicolumn{1}{c}{SSIM$\uparrow$} & \multicolumn{1}{c}{LPIPS$\downarrow$} & \multicolumn{1}{c}{PSNR$\uparrow$} & \multicolumn{1}{c}{SSIM$\uparrow$} & \multicolumn{1}{c}{LPIPS$\downarrow$} \\
\midrule
\small
NeRF-T &        21.84       &      0.69              &       0.37           &               12.33  &          0.49            &        0.65             &       21.98            &             0.69        &        0.46            \\
\small
HyperNeRF &    16.43            &     0.43         &    0.40            &     16.81            &    0.41        &          0.56        &      16.04           &           0.38      &         0.62           \\
\midrule
\small
Ours      &        \bf{23.98}                  &       \bf{0.77}              &                \bf{0.26}      &   \bf{24.71}            &           \bf{0.80}               &       \bf{0.26}                    &      \bf{25.43}          &            \bf{0.79}              &       \bf{0.31}              \\
\bottomrule
\\ 
\end{tabular}

\begin{tabular}{lccccccccc}
\toprule
          & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Bike\end{tabular}}  & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Jogging\end{tabular}}   & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Lab\end{tabular}} \\
          & \multicolumn{1}{c}{PSNR$\uparrow$} & \multicolumn{1}{c}{SSIM$\uparrow$} & \multicolumn{1}{c}{LPIPS$\downarrow$} & \multicolumn{1}{c}{PSNR$\uparrow$} & \multicolumn{1}{c}{SSIM$\uparrow$} & \multicolumn{1}{c}{LPIPS$\downarrow$} & \multicolumn{1}{c}{PSNR$\uparrow$} & \multicolumn{1}{c}{SSIM$\uparrow$} & \multicolumn{1}{c}{LPIPS$\downarrow$} \\
\midrule
\small
NeRF-T &   21.16     &      0.71         &     0.36         &     20.63        &       0.53         &         0.49        &     20.52         &    0.75      &       0.39        \\
\small
HyperNeRF &     17.64     &   0.42   &      0.43  &       18.52          &  0.39    & 0.52               &      16.75      &    0.51      &     0.23          \\
\midrule
\small
Ours      &     \bf{25.52}          &     \bf{0.82}        &      \bf{0.23}         &     \bf{22.68}    &          \bf{0.67}      &         \bf{0.32}          &   \bf{24.93}      &        \bf{0.85}          &       \bf{0.21}        \\
\bottomrule
\end{tabular}

\end{center}
\caption{
{\bf Novel view synthesis comparison --} We report the quantitative results on test views.
Our method achieves the best rendering quality across all scenes and all metrics by a large margin.
Notice that the numbers for ours method depends on the estimated human pose.
}
\label{tab:novel_view}
\end{table}


    


